Audio-visual Generalized Zero-shot Learning the Easy Way

Audio-visual generalized zero-shot learning is a rapidly advancing domain that seeks to understand the intricate relations between audio and visual cues within videos. The overarching goal is to leverage insights from seen classes to identify instances from previously unseen ones. Prior approaches primarily utilized synchronized auto-encoders to reconstruct audio-visual attributes, which were informed by cross-attention transformers and projected text embeddings. However, these methods fell short of effectively capturing the intricate relationship between cross-modal features and class-label embeddings inherent in pre-trained language-aligned embeddings. To circumvent these bottlenecks, we introduce a simple yet effective framework for Easy Audio-Visual Generalized Zero-shot Learning, named EZ-AVGZL, that aligns audio-visual embeddings with transformed text representations. It utilizes a single supervised text audio-visual contrastive loss to learn an alignment between audio-visual and textual modalities, moving away from the conventional approach of reconstructing cross-modal features and text embeddings. Our key insight is that while class name embeddings are well aligned with language-based audio-visual features, they don't provide sufficient class separation to be useful for zero-shot learning. To address this, our method leverages differential optimization to transform class embeddings into a more discriminative space while preserving the semantic structure of language representations. We conduct extensive experiments on VGGSound-GZSL, UCF-GZSL, and ActivityNet-GZSL benchmarks. Our results demonstrate that our EZ-AVGZL achieves state-of-the-art performance in audio-visual generalized zero-shot learning.

==> 0-space-saving.tex <==
%% Shrink space around figures.
%% This beats manually adding negative \vspace commands everywhere.
\setlength{\textfloatsep}{2pt}
% \setlength{\textfloatsep}{20pt plus 2pt minus 4pt}
% \setlength{\textfloatsep}{16pt plus 2pt minus 4pt}
% \setlength{\textfloatsep}{6pt plus 2pt minus 4pt}
% \setlength{\dbltextfloatsep}{0pt}
% \setlength{\intextsep}{0pt}
\captionsetup{font=footnotesize}
\setlength{\abovecaptionskip}{2pt}
\setlength{\belowcaptionskip}{5pt}
% \setlength{\parskip}{0pt}
%% around equations
\setlength{\abovedisplayskip}{2pt}
\setlength{\belowdisplayskip}{2pt}
\setlength\abovedisplayshortskip{1pt}
\setlength\belowdisplayshortskip{1pt}

%% The wrapfigure environment is also a good way to use less space for a small figure.
%% It is finicky.
%% See: http://en.wikibooks.org/wiki/LaTeX/Floats,_Figures_and_Captions#Wrapping_text_around_figures

%% Shrink space around enumerate and itemize
%% From: http://tex.stackexchange.com/questions/10684/vertical-space-in-lists
%\usepackage{enumitem}
%% Set it globally:
% \setlist{nosep} % or \setlist{noitemsep} to leave space around whole list
% \setlist{itemsep=1pt, topsep=3pt}
%% Or locally:
% \begin{enumerate}[itemsep=1pt, topsep=12pt, partopsep=0pt]

%% Less space around titles.
%% From: http://tex.stackexchange.com/questions/4999/change-whitespace-above-and-below-a-section-heading
% \usepackage[medium,compact]{titlesec}
%% or
% \usepackage{titlesec}
% \titlespacing*{\section}{0pt}{*1}{*1}

%% Shrink the \paragraph command.
\renewcommand{\paragraph}[1]{\noindent {\bf #1}}

%% Allow Latex to use a smaller minimum spacing between lines.
%\renewcommand{\baselinestretch}{0.97}
% \renewcommand{\baselinestretch}{0.99}

%% Shrink space between lines. You probably want to prefer baselinestretch in general.
%% From: http://tex.stackexchange.com/questions/23824/6-lines-in-one-inch
%% 6 lines in one inch with an 11pt font:
% \linespread{0.950}
% \linespread{0.909}
\linespread{0.909}
%\linespread{1}

%% Shrink the spacing between lines in just the bibliography. This is good.
% \usepackage{setspace}

%% Then wrap the bibliography in a \begin{spacing}. You can wrap any section like this.
% \begin{spacing}{0.9}
% \bibliographystyle{...}
% \bibliography{refs}
